Epidemics on Networks

Despite centuries of work on containment and mitigation strategies, infectious diseases are still a major problem facing humanity. This work is concerned with simulating heterogeneous contact structures and understanding how the structure of the underlying network affects the spread of the disease. For example, it has been empirically demonstrated and validated that scale free networks do not have an epidemic threshold. Understanding the relationship between network structure and disease dynamics can help to develop better mitigation strategies and more effective interventions.

==> misc.tex <==
\clearpage
\section{Open Questions}
\begin{enumerate}
\item How long will the COVID-19 pandemic last and when will we end up in a more ore less steady state?
\item How can we model the model the number of hospitalised and sever cases depending on the number of susceptible, infected, recovered, vaccinated people?
\item How common will reinfection be and how long will immunity last?
\item How will new virus variants affect the development of the pandemic?
\item What proportion of transmission do asymptomatic people account for?
\item How can we identify (potential) superspreaders?
\item Where do most COVID-19 infections happen? (For example the COVID certificate will be less efficient when many infections happen in a private context where there is no certificate requirement)
\item How high is the true basic reproduction number $R_0$ in a completely susceptible population?
\item How long will the pandemic probably last until it reaches a stable state?
\item One of the most important probems in epidemiology is to ascertain whether this termination occurs only when no susceptible individuals are left, or whether the interplay of the various factors of infectivity, recovery and mortality, may result in termination, whilst many susceptible individuals are
still present in the unaffected population \cite{WilliamKermack1927}
\end{enumerate}

\begin{center}
\captionof{table}{Analysed networks}
\begin{tabular}{p{1.2cm} p{1.05cm} p{2.1cm} p{1.4cm}}
\hline
Network &$<k>$ &Scale-free &Density\\
\hline
1 (BA) & 9.95 &True (2.72)& 0.9960\%\\ 
2 (ER) & 9.86 &False (8.22)& 0.9872\%\\  
3 (WS) & 10.0 &False (10.13)& 1.0010\%\\  
 4 (FF) & 43.69 & True (2.51) & 1.0820\%\\ 
 5 (SE) & 4.67 & True (2.87) & 0.0279\%\\  
 6 (CT) & 6.46 & False (3.0) & 1.5490\%   
\label{tab:networks}
\end{tabular}
\end{center}

























\subsection{Interventions}
Interventions can be implemented top-down or at the individual level, in order to curb the spreading dynamics
\begin{enumerate}
    \item Social Distancing
    \item Masks
    \item Lockdowns
    \item Travel Restrictions
    \item COVID Pass
    \item Vaccinations
    \item Testing
\end{enumerate}

 
